FederBoost: Private Federated Learning for GBDT

Federated Learning (FL) has been an emerging trend in machine learning and artificial intelligence. It allows multiple participants to collaboratively train a better global model and offers a privacy-aware paradigm for model training since it does not require participants to release their original training data. However, existing FL solutions for vertically partitioned data or decision trees require heavy cryptographic operations. In this paper, we propose a framework named FederBoost for private federated learning of gradient boosting decision trees (GBDT). It supports running GBDT over both vertically and horizontally partitioned data. Vertical FederBoost does not require any cryptographic operation and horizontal FederBoost only requires lightweight secure aggregation. The key observation is that the whole training process of GBDT relies on the ordering of the data instead of the values. We fully implement FederBoost and evaluate its utility and efficiency through extensive experiments performed on three public datasets. Our experimental results show that both vertical and horizontal FederBoost achieve the same level of accuracy with centralized training where all data are collected in a central server, and they are 4-5 orders of magnitude faster than the state-of-the-art solutions for federated decision tree training; hence offering practical solutions for industrial applications.

==> sections/background.tex <==
% \subsection{Background}
\subsection{Gradient boosting decision tree (GBDT)}
\label{sec:GBDT}

A decision tree is a tree-like model for machine learning predictions. 
It consists of nodes and edges: 
each internal node represents a ``test'' on a feature; 
each edge represents the outcome of the test;
and each leaf node represents the prediction result.
The path from root to a leaf represents a prediction rule.


\begin{figure}[htbp]
\centering
\includegraphics[width=0.46\textwidth]{./sections/plot/tree.png}
\caption{An example of GBDT.}
\label{fig:tree}
\end{figure}


Gradient boosting decision tree (GBDT) is a boosting-based machine learning algorithm that ensembles a set of decision trees\footnote{In fact, it is a regression tree; we abuse the notion here.}~\cite{XGBoost}.
%It is also one of the most popular choices [7] in data analytics competitions such as Kaggle and KDDCup, and has been widely used in both academia and industry. 
Figure~\ref{fig:tree} shows an example of GBDT: in each tree, the input $\x$ is classified to one leaf node that predicts the input with a weight; then it sums the predictions of all trees and gets the final prediction: 
\begin{equation}
\label{equ:prediction}
    \hat{y} = \sum_{t=1}^{T}f_{t}(\x)
\end{equation}
where $T$ denotes the number of trained decision trees and $f_t(\x)$ denotes the prediction result of the $t$th tree.
For classification, it calculates $p = \mathrm{sigmoid}(\hat{y})$ and determines its predicted class based on $p$. 
 

Next, we explain how a GBDT training algorithm works given a dataset $\textbf{X} \in \mathbb{R}^{n\times m}$ that consists of $n$ samples and $m$ features.
It first initializes the prediction result $\hat{y}^0_i$ for each sample with random values.
Then, it trains the $t$th decision tree as follows:
\begin{enumerate}
\item For each sample, calculate the {\em first-} and {\em second-order gradient}: 

\begin{equation}
\label{equ:gh}
\begin{split}
g_i=\partial_{\hat{y_i}^{(t-1)}}L(y_i,\hat{y_i}^{(t-1)}), \\
h_i=\partial^2_{\hat{y_i}^{(t-1)}}L(y_i,\hat{y_i}^{(t-1)}) 
\end{split}
\end{equation}

where $\hat{y_i}^{(t-1)}$ is the prediction result aggregated from previous trees, $y_i$ is the real label, and $L(y_i,\hat{y_i}^{(t-1)})$ is the loss function.
The binary cross entropy loss function is typically used as a loss function.
%\footnote{We use $g_i = \hat{y}_i - y_i$ and $h_i = \hat{y}_i(1-\hat{y}_i)$ for the classification problems in our experiments.}. 

%In this paper, we use the binary cross entropy loss function $L(y_i,\hat{y_i}^{(t-1)})$. \todo{Give reference!}
% \begin{equation}
% \begin{split}
%     L(y_i,\hat{y}^{(t-1)})=&-[y_i log(\frac{1}{1+e^{-w_i})\\ &+(1-y_i)log(\frac{e^{-\hat{y_i}^{(t-1)}}}{1+e^{-w_i)]\\e
% \end{split}
% \end{equation}
% We get $g_i = \frac{1}{1+e^{-w_i}} - y_i$ and $h_i =\frac{e^{-w_i}}{(1+e^{w_i})^2}$.

\item Run the following steps for each node of the tree from root to leaf:
\begin{enumerate}
\item For each feature, find the best split of the samples that maximize the following function:
\begin{equation}
\label{equ:split1}
\begin{aligned}
\mathcal{L_\mathit{split}}=&\frac{1}{2} [\frac{(\sum_{i \in I_L} g_i)^2}{\sum_{i \in I_L} h_i +\lambda}\\
+&\frac{(\sum_{i \in I_R} g_i)^2}{\sum_{i \in I_R} h_i +\lambda}+\frac{(\sum_{i \in I} g_i)^2}{\sum_{i \in I} h_i +\lambda}]
\end{aligned}
\end{equation}
where $\lambda$ is a hyper-parameter, $I_L$ denotes the samples divided into the left child node, $I_R$ denotes the samples divided into the right child node, and $I$ denotes all samples in the current node.
The samples in $I_L$, $I_R$ and $I$ are in a sorted order of their corresponding feature values.
\item Choose the feature with the maximal $\mathcal{L_\mathit{split}}$ for the current node and split the samples accordingly.
\end{enumerate}
\item The weight of each leaf is computed by the following function:
\begin{equation}
\label{equ:weight}
    w=-\frac{\sum_{i \in I} g_i}{\sum_{i \in I} h_i +\lambda}
\end{equation}
This is the prediction result %$\hat{y}^{(t)}$ 
for the samples falling into this leaf.
\end{enumerate}

Most GBDT frameworks accelerate the training process by building a {\em gradient histogram} for each feature to summarize the gradient statistics; the best split can be found based on the histograms.
%put the samples of each feature into buckets, aggregate the statistics in each bucket, and find the best split of buckets based on the aggregated statistics.
More specifically, for each feature, the training algorithm sorts the samples based on their feature values as before. 
Then, it partitions the samples and puts them into $q$ buckets.
For each {\em bucket}, it calculates $G = \sum_{i \in \mathit{bucket}} g_i$ and $H = \sum_{i \in \mathit{bucket}} h_i$.
The gradient histogram for a feature consists of these $G$s and $H$s of all buckets.
Then, the best split for a feature can be found by maximizing:
%and uses them for finding the splits:
\begin{equation}
\label{equ:split2}
\mathcal{L_\mathit{split}}=\frac{1}{2} [\frac{(\sum_{i \in I_L} G_i)^2}{\sum_{i \in I_L} H_i +\lambda}+\frac{(\sum_{i \in I_R} G_i)^2}{\sum_{i \in I_R} H_i +\lambda}+\frac{(\sum_{i \in I} G_i)^2}{\sum_{i \in I} H_i +\lambda}]
\end{equation}
Empirically, 20 buckets are used in popular GBDT frameworks~\cite{DimBoost,vero}.
The split finding algorithm is depicted in Algorithm~\ref{alg:split}.

% \floatname{algorithm}{Algorithm}
% \renewcommand{\algorithmicrequire}{\textbf{Input}:}
% \renewcommand{\algorithmicensure}{\textbf{Output}:}
% \renewcommand{\algorithmiccomment}[1]{$\triangleright$ #1}
% \begin{algorithm}[htb]
% \caption{Split Finding}
% \begin{algorithmic}[1]
% \label{alg:split}
% \REQUIRE  $\{G_{1}, ..., G_{d}\}$, $\{H_{1}, ..., H_{d}\}$
% %$d$ buckets sorted in order, each with $G$ and $H$
% \ENSURE Split with max score
% \STATE $\GG \gets \sum_{i=1}^dG_{i}$, $\HH \gets \sum_{i=1}^dH_{i}$
% \STATE $\GG_L \gets 0$, $\GG_R \gets 0$

% \FOR{$i = 1 \to d$}
% \STATE $\GG_L \gets \GG_L + G_{i}$,
% $\HH_L \gets \HH_L + H_{i}$
% \STATE $\GG_R \gets \GG - \GG_L$, 
% $\HH_R \gets \HH - \HH_L$

% \STATE $\mathit{score}\gets max(\mathit{score},\frac{G_L^2}{ H_L +\lambda}+\frac{G_R^2}{H_R +\lambda}+\frac{G^2}{ H +\lambda})$
% \ENDFOR
% %\STATE $\mathit{score}_\mathit{feature} \gets max(\mathit{score}_\mathit{feature}, \mathit{score}_\mathit{split})$

% \end{algorithmic}
% \end{algorithm}
%\floatname{algorithm}{Algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input}:}
\renewcommand{\algorithmicensure}{\textbf{Output}:}
\renewcommand{\algorithmiccomment}[1]{$\triangleright$ #1}
\begin{algorithm}
\caption{Split Finding}
\label{alg:split}
\small
\KwIn{  $\{G_{1}, ..., G_{q}\}$, $\{H_{1}, ..., H_{q}\}$}
%$d$ buckets sorted in order, each with $G$ and $H$
\KwOut {split with max score}
$\GG \gets \sum_{i=1}^qG_{i}$, $\HH \gets \sum_{i=1}^qH_{i}$

$\GG_L \gets 0$, $\GG_R \gets 0$

\For{$i = 1 \to q$}{
$\GG_L \gets \GG_L + G_{i}$,
$\HH_L \gets \HH_L + H_{i}$

$\GG_R \gets \GG - \GG_L$, 
$\HH_R \gets \HH - \HH_L$

$\mathit{score}\gets max(\mathit{score},\frac{G_L^2}{ H_L +\lambda}+\frac{G_R^2}{H_R +\lambda}+\frac{G^2}{ H +\lambda})$
}
%\STATE $\mathit{score}_\mathit{feature} \gets max(\mathit{score}_\mathit{feature}, \mathit{score}_\mathit{split})$
\end{algorithm}

%To train the model, it adds the tree $f_t$ one by one. At the $t^{th}$ iteration, the loss is as followed
%$\mathcal{L_\mathit{split}} = \sum_{i=1}^{n}[l(y_i,\hat{y_i}^{(t-1)}+g_if_t(x_i)+\frac{1}{2}h_if_t^2(x_i)]+\omega(f_t)$,
%where $\omega(f_t)=\gamma T+\frac{1}{2}\lambda||w||^2,g_i=\partial_{\Breve{y}^{(t-1)}}l(y_i,\Breve{y}^{(t-1)}),h_i=\partial^2_{\Breve{y}^{(t-1)}}l(y_i,\Breve{y}^{(t-1)})$

\subsection{Federated learning}
\label{sec:fl}

The goal of federated learning (FL) is to enable multiple participants to contribute various training data to train a better model.
It can be roughly classified into two categories~\cite{yang2019federated}: horizontal FL and vertical FL. 

One horizontal FL method~\cite{mcmahan17a} proposed by Google is to distribute the model training process 
of a deep neural network 
across multiple participants by iteratively aggregating the locally trained models into a joint global one. 
%Federated learning allows multiple participants to jointly train a shared model by only communicating model parameters~\cite{mcmahan17a}.
%It can effectively save network bandwidth given that model parameters are significantly smaller than training data. 
There are two types of roles in this protocol: a parameter server and $l$ participants $\Cli$s. 
%The whole model training process progresses in iterations. 
In the beginning, the parameter server initializes a model  with random values and sends it to all $\Cli$s.
In each iteration, each $\Cli_j$ ($j \in [1, l]$) trains the received model  with its local data, and sends parameter server its gradients.
%model updates $\Delta \M_{j}^i$, 
%which are the differences between its locally trained model and $\M^{i-1}$. 
The parameter server aggregates the received gradients and updates the global model.
% \begin{center}
% %\label{equ:federated}
% $\theta^{i} = \theta^{i-1} + \frac{\eta}{l} \sum_{j=1}^l \g^{i}_j$, 
% \end{center}
% where $\eta$ is the global learning rate.

This elegant paradigm {\em cannot} be directly applied to vertical FL, where participants have different feature spaces so that
they cannot train models locally.
Furthermore, the FL research committee is focusing on neural networks and less attention has been paid to decision trees.


\subsection{Secure aggregation}
\label{sec:aggregation}


Bonawitz, et al.~\cite{bonawitz2017practical} propose a {\em secure aggregation} protocol to protect the local gradients in Google's horizontal FL.
Specifically, they use pairwise additive masking to protect participants' local gradients, 
and have the parameter server aggregate the masked inputs. 
The masks are generated by a pseudorandom generator (PRG) using pairwise shared seeds and will get canceled after aggregation.
The seeds are shared via threshold secret sharing so that dropped-out participants can be handled.
A malicious server can lie about whether a $\Cli_i$ has dropped out, thereby asking all other participants to reveal their shares of $\Cli_i$'s masks.
To solve this issue, they introduce a {\em double masking} scheme requiring each participant to add another mask to its input and share this mask as well.
The server can request either a share of the pairwise mask (which will get canceled if no one drops) or a share of the new mask;
an honest participant will never reveal both shares for the same participant to the server.
In this paper, we assume the participants are large organisations and they will not drop out in the middle of the protocol, thereby we significantly simplify the secure aggregation protocol.


%Notice that a malicious server can lie about whether a client $\Cli_i$ has dropped out, thereby asking all other clients to reveal their shares of $\Cli_i$'s masks.
%To solve this issue, they introduce a {\em double masking} scheme requiring each client to add another mask to its input and share this mask as well.
%The server can request either a share of the pairwise mask (which will get canceled if no one drops) or a share of the new mask;
%an honest client will never reveal both shares for the same client to the server.


\subsection{Differential privacy}
\label{sec:dp}
% The successful deployment of various data analysis techniques has let people realized the importance of detailed data, but also raised privacy concerns. Anonymity is not an ideal solution because it has been shown that such data could be de-anonymized by linking them with publicly available data~\cite{narayanan2006break}.

Given a set of input data and an analysis task to perform, the goal of {\em differential privacy}~\cite{differential} is to permit statistical analysis while  protecting each individual's data.
It aims to ``hide'' some input data from the output: by looking at the statistical results calculated from the input data, one cannot tell whether the input data contains a certain record or not. 
%Formally, differential privacy is defined as below:



\begin{definition}[$(\varepsilon, \delta)$-Differential Privacy~\cite{differential}]
A randomized algorithm $\mathcal{M}$ with domain $\mathbb{N}^{|\mathcal{X}|}$ is $(\varepsilon,\delta)$-differentially private if for all $\mathcal{S} \subseteq \mathtt{Range}\left(\mathcal{M}\right)$ and for any neighboring datasets $D$ and $D'$:
\begin{equation*}
    \Pr[\mathcal{M}(D) \in \mathcal{S}] \leq e^\varepsilon\Pr[\mathcal{M}(D')\in \mathcal{S}] + \delta.
\end{equation*}
\end{definition}

It guarantees that, by examining the outputs $\mathcal{M}(D)$ and $\mathcal{M}(D')$, one cannot reveal the difference between $D$ and $D'$.
Clearly, the closer $\epsilon$ is to $0$, the more indistinguishable $\mathcal{M}(D)$ and $\mathcal{M}(D')$ are, and hence the better the privacy guarantee.
%The notion of \textit{adjacent datasets} may differ depending on applications.
This nice property provides {\em plausible deniability} to the data owner, because the data is processed behind a veil of uncertainty.
%Previous work mostly explore the setting where $d$ and $d'$ differ by a single record, which is referred as \textit{record-level differential privacy}.



==> sections/security.tex <==
\subsection{Security Analysis of Vertical $\name$}
\label{sec:vertical_analysis}
\Paragraph1{$\Cli_i$'s security.} During training, the active participant $\Cli_l$ {\em only} learns the order of buckets for each feature behind a veil of uncertainty:
each sample has a probability of $p=\frac{q-1}{e^{\epsilon}+q-1}$ to be placed in a wrong bucket.
When $\epsilon=2$ and $q=16$, $p$ is approximately $67\%$.

During prediction, $\Cli_l$ only learns the comparison result of each node, but nothing else. 
We consider a more powerful $\Cli_l$, who can control the input $\x$ to the prediction phase. 
Nevertheless, the best $\Cli_l$ can do is to use binary search to learn the threshold value of each node. 
Recall that the threshold value could be any value between the boundaries of two buckets,
$\Cli_l$ learns nothing about the samples themselves.

The above argument remains true even if $\Cli_l$ colludes with other $l-1$ passive participants. 
\Paragraph{$\Cli_l$'s security.}
During the whole training process, the only information a passive party $\Cli_i$ learns is the split information sent by $\Cli_l$ (line 21 of protocol 2),
which indicates how the buckets are split into left and right, leading to the maximal $L_{split}$ in equation 2.5. 
However, such information is not enough for $\Cli_i$ to infer anything about $G_i$ and $H_i$, hence the labels $y$s and prediction results $\hat{y}$ are kept private. 

Suppose $\Cli_l$ also holds a feature $\x^l$.
If $\Cli_l$'s feature $\x^l$ was selected by a tree node, 
the holders of child-node learn that the samples assigned to left is smaller than the samples assigned to right.
Nevertheless, such information is also protected by differential privacy.

During prediction, each $\Cli_i$ only compares its threshold value with the corresponding feature of $\x$, and learns exactly nothing.

The above argument remains true even if $\Cli_i$ colludes with other $l-2$ passive participants. 
\subsection{Security Analysis of Horizontal $\name$}
\label{sec:horizontal_analysis}
\Paragraph1{$\Cli_i$'s security.} 
There are two places for potential information leakage:
\begin{itemize}
    \item During quantile lookup, $\Cli_i$ inputs $n'_i$ to secure aggregation (line 9 of Protocol 3). 
    \item During tree construction, $\Cli_i$ inputs $G^i_{j,k}$ and $H^i_{j,k}$ to secure aggregation (line 20 of Protocol 4).
\end{itemize}

Both inputs are protected by secure aggregation.
Although $\Cli_l$ can collude with $\tau-1$ passive participants, it still cannot learn anything beyond the sum of $l-\tau$ participants' inputs.  
\Paragraph{$\Cli_l$'s security.}
There are again two places for potential information leakage:
\begin{itemize}
    \item During quantile lookup, $\Cli_l$ sends $Q_j$ to other $\Cli$s (line 5 of Protocol 3). 
    \item During tree construction, $\Cli_l$ sends $\mathit{split}_{j}$ to other $\Cli$s (line 24 of Protocol 4).
\end{itemize}
Notice that $Q_j$ is calculated based on $n'$ and $\mathit{split}_j$ is calculated based on $G^i_j$ and $H^i_j$.
Therefore, the information leakage of $\Cli_l$ will not be larger than $\Cli_i$ ($\Cli_i$'s security was proved above).

